Axiomatising Infinitary Probabilistic Weak Bisimilarity of Finite-State Behaviours

In concurrency theory, weak bisimilarity is often used to relate processes exhibiting the same observable behaviour. The probabilistic environment gives rise to several generalisations; we study the infinitary semantics, which abstracts from a potentially unbounded number of internal actions being performed when something observable happens. Arguing that this notion yields the most desirable properties, we provide a sound and complete axiomatisation capturing its essence. Previous research has failed to achieve completeness in the presence of unguarded recursion, as only the finitary variant has been axiomatised, yet.

==> sections/definitions/weak-transitions/weaktran <==
\begin{center}
\hfill
	\AxiomC{}
	\UnaryInfC{$\mu \wtrans{}_\convex^\finitary \mu$}
	\bottomAlignProof
	\DisplayProof
\hfill
	\AxiomC{$\mu \trans\tau_{\chR{\convex}} \nu$}
	\UnaryInfC{$\mu \wtrans{}_\convex^\finitary \nu$}
	\bottomAlignProof
	\DisplayProof
\hfill
	\AxiomC{$\forall i.\; \mu_i \wtrans{}_\convex^\finitary \nu_i$}
	\RightLabel{$\sum_i p_i \leq 1$}
	\UnaryInfC{$\sum_i p_i \mu_i \wtrans{}_\convex^\finitary \sum_i p_i \nu_i$}
	\bottomAlignProof
	\DisplayProof
\hspace*{\fill}\null\\[1.8ex]
\hfill
	\AxiomC{$\mu \wtrans{}_\convex^\finitary \gamma$}
			\AxiomC{$\gamma \wtrans{}_\convex^\finitary \nu$}
	\BinaryInfC{$\mu \wtrans{}_\convex^\finitary \nu$}
	\DisplayProof
\hspace*{\fill}
\end{center}

